Demystifying MPNNs: Message Passing as Merely Efficient Matrix Multiplication

While Graph Neural Networks (GNNs) have achieved remarkable success, their design largely relies on empirical intuition rather than theoretical understanding. In this paper, we present a comprehensive analysis of GNN behavior through three fundamental aspects: (1) we establish that \textbf{$k$-layer} Message Passing Neural Networks efficiently aggregate \textbf{$k$-hop} neighborhood information through iterative computation, (2) analyze how different loop structures influence neighborhood computation, and (3) examine behavior across structure-feature hybrid and structure-only tasks. For deeper GNNs, we demonstrate that gradient-related issues, rather than just over-smoothing, can significantly impact performance in sparse graphs. We also analyze how different normalization schemes affect model performance and how GNNs make predictions with uniform node features, providing a theoretical framework that bridges the gap between empirical success and theoretical understanding.

==> 6_experi.tex <==
\section{Experiments}

% \subsection{$k$-layer GCN with A VS. $1$-layer GCN with $A^k$}

In this section, we will use widely-adopted real-world datasets to test performance of $k$-layer GCN with $A$ VS. $1$-layer GCN with $A^k$. More details about the datasets are presented in Appendix \ref{ap:data}.

% We will first experiment on GCN without self-loops, then on GCN with selfloops.
% \subsection{GCN without self-loops}
% GCN without self-loops don't suffer from over-smoothing even with up to 50 layers as shown in Fig. \ref{fig:chame&squi_2hop}, while generally GNN is believed to suffer from over-smoothing within 5 layers \cite{liDeeperInsightsGraph2018}.

% This coincides with our previous theoretical proof that adding selfloops would cause coexistence of different hops of neighbors, which might lead to over-smoothing.

% \input{figs/fig_chame_2hop}


% \subsection{GCN with selfloops}
% The experimental results on CoraML and CiteSeer dataset is shown in Fig. \ref{fig:cite_3} and \ref{fig:cora_3}. Although they are equivalent in Universal Approximation Theorem, the performance have great difference as more hops of neighbors are aggregated. The performance of $1$-layer GCN of $A^k$ tends to be stable as $k$ increases, while the performance of $k$-layer GCN of $A$ deteriorates greatly 
%  as layers go deeper.
%  Since $1$-layer GCN of $A^k$ and $k$-layer GCN of $A$ involves with the same depth of neighborhood, 
%  it is not over-smoothing that cause the worse performance, it is actually vanishing gradients. This is contrary to the commonly held belief that over-smoothing causes the worse performance of deep GNNs. 

% As this is directed graph and the aggregation is also directed, although the GCN used is adding selfloops, the density of graph is quite low, as shown in Fig. \ref{fig:cite_3} and \ref{fig:cora_3}.

% This shows that even adding selfloops, the deteriation of performance as layer goes deeper is not necessarily caused by over-smoothing.

\input{figs/cite}
\input{figs/cora}
\input{figs/pubmed}

\input{figs/wikics}

\input{figs/tel}





==> bin.tex <==
% Formally, the $k$-th layer of a GNN is
% \begin{equation}
    
% \end{equation}
% \begin{equation}
% \label{eq:total2-1}
%     a_v^{(k)} = AGGR^{(k)} \big( \{ h_u^{(k-1)}: u \in \mathcal{N}(v) \} \big), 
% \end{equation}
% \begin{equation}
% \label{eq:total2-2}
%     h_v^{(k)}= COMB^{(k)} \big( h_v^{(k-1)}, a_v^{(k)}  \big),
% \end{equation}
% where $h_v^(k)$ is the feature vector of node $v$ at the $k$-th iteration/layer. We initialize $h_v^{(0)}= X_v$, and $\mathcal{N}(v)$ is a set of nodes adjacent to $v$, generally 1-hop neighbors, may expand to k-hop neighbors in Higher-Order Neighborhood Aggregation models. The difference of GNN variants lies in the choice of $AGGR^{(k)}(\cdot)$ and $COMB^{(k)}(\cdot)$. 

% \begin{equation}
%   h_v^{(k)} = \text{ReLU}\left( W \cdot \text{MEAN} \left\{ h_u^{(k-1)} \mid \forall u \in \mathcal{N}(v) \cup \{v\} \right\} \right),
% \end{equation}

\begin{equation}
    H^{(k+1)} = \sigma(W_1^{(k)}W_n \odot A H^{(k)} + W_2^{(k)}H^{(k)})   \\
    = \sigma((W_1^{(k)}W_n \odot A + W_2^{(k)})H^{(k)})
\end{equation}
which can be simplified as 

\footnote{Many papers \cite{mauryaSimplifyingApproachNode2022} write $H^{(k+1)} = \sigma(\widetilde{A}_{\text{sym}} H^{(k)}W^{(k)})$, but swapping the order of aggregation and the fully connected step has little impact on predictions.}

\\
              &= \sigma\big((W_1^{(k)} W_n \odot A + W_2^{(k)}I) H^{(k)}\big)

==> figs/cite_1.tex <==
\begin{figure}
    \centering
\captionsetup{font=small}

% \vskip 0.15in
    \includegraphics[width=0.8\linewidth]{figs/citeseer+a+accuracy+trend.pdf}
    % \includegraphics[width=\linewidth]{figs/CiteSeer with At: Accuracy trend with growing layer or k in k-hop neighbors.pdf}
    % \includegraphics[width=\linewidth]{figs/CiteSeer with Undirect: Accuracy trend with growing layer or k in k-hop neighbors.pdf}

    % \includegraphics[width=\linewidth]{figs/CiteSeer with A3: Accuracy trend with growing layer or k in k-hop neighbors.pdf}
    % \vspace{-2em} % Adjust the value
    \vskip -0.15in
    
\caption{Comparison of different GCN architectures on CiteSeer: k-layer GCN (blue), 1-layer GCN with k-hop neighbors (red), and k-hop neighbors with (k-1) linear layers (green). The black line shows the density of k-hop adjacency matrix.}

    \label{fig:cite_1}
\end{figure} 

==> figs/cora_1.tex <==
\begin{figure}
    \centering
        \captionsetup{font=small}

% \vskip -0.15in
    \includegraphics[width=0.8\linewidth]{figs/CoraML+A.pdf}
    % \includegraphics[width=\linewidth]{figs/CoraML with At: Accuracy trend with growing layer or k in k-hop neighbors.pdf}
    % \includegraphics[width=\linewidth]{figs/CoraML with A3: Accuracy trend with growing layer or k in k-hop neighbors.pdf}
    % \includegraphics[width=\linewidth]{figs/CoraML with Undirect: Accuracy trend with growing layer or k in k-hop neighbors.pdf}
    % \vspace{-1em} % Adjust the value
    \vskip -0.15in
    \caption{Comparison of different GCN architectures on CoraML: k-layer GCN (blue), 1-layer GCN with k-hop neighbors (red), and k-hop neighbors with (k-1) linear layers (green). The black line shows the density of k-hop adjacency matrix.}

    \label{fig:cora_1}
\end{figure}

==> figs/pubmed_1.tex <==
\begin{figure}
    \centering
    \captionsetup{font=small}

    \includegraphics[width=0.8\linewidth]{figs/PubMed+A.pdf}
    % \includegraphics[width=\linewidth]{figs/PubMed with At: Accuracy trend with growing layer or k in k-hop neighbors.pdf}
    % \includegraphics[width=\linewidth]{figs/PubMed with Undirect: Accuracy trend with growing layer or k in k-hop neighbors.pdf}
    \vspace{-1em} % Adjust the value
    \caption{Comparison of different GCN architectures on PubMed: k-layer GCN (blue), 1-layer GCN with k-hop neighbors (red), and k-hop neighbors with (k-1) linear layers (green). The black line shows the density of k-hop adjacency matrix.}
    \label{fig:pubmed_1}
\end{figure} 

==> proof_klayer.tex <==
\subsection{Node representation after $2$-lay GNN}

According to Eq. \ref{eq:sum}, for general GNNs, the layer-wise propagation output is:
\begin{equation}
h_i^{(k+1)} = \sigma \left( W_1^{(k)} h_i^{(k)} + W_2^{(k)} \sum_{j \in \mathcal{N}(i)} h_j^{(k)} + b^{(k)} \right)
% \label{eq:sum}
\end{equation}

the node representation after 
1-layer GNN:
\begin{align}
h_i^{(1)} = \sigma \left( W_1^{(0)} h_i^{(0)} + W_2^{(0)} \sum_{j \in \mathcal{N}(i)} h_j^{(0)} + b^{(0)} \right)
% \tag{1}
\end{align}

2-lay GNN:
\begin{equation}
\label{eq:proof_2layer}
    h_i^{(2)} = \sigma \left( W_1^{(1)} h_i^{(1)} + W_2^{(1)} \sum_{j \in \mathcal{N}(i)} \sigma \left( W_1^{(0)} h_j^{(0)} + W_2^{(0)} \sum_{k \in \mathcal{N}(j)} h_k^{(0)} + b^{(0)} \right) 
            + b^{(1)} \right) \\
\end{equation}

Thanks to the universal approximation theorem (UAT) \cite{HornikKurt1989Mfna, hornikApproximationCapabilitiesMuitilayer}, Eq. \ref{eq:proof_2layer} can be further simplified as:
\begin{align}
\label{eq:proof_2layer}
    h_i^{(2)} &= \sigma \left( W_1^{(1)} h_i^{(1)} + W_2^{(1)} \sum_{j \in \mathcal{N}(i)} \left( W_1^{(0)} h_j^{(0)} + W_2^{(0)} \sum_{k \in \mathcal{N}(j)} h_k^{(0)} + b^{(0)} \right)  + b^{(1)}\right) \\
    &\quad = \sigma \left( W_1^{(1)} h_i^{(1)} + W_2^{(1)} \sum_{j \in \mathcal{N}(i)} W_1^{(0)} h_j^{(0)} + W_2^{(1)} W_2^{(0)} \sum_{j \in \mathcal{N}(i)} \sum_{k \in \mathcal{N}(j)} h_k^{(0)} + W_2^{(1)} |\mathcal{N}(i)| b^{(0)} + b^{(1)} \right) \\
    &\quad = \sigma \left( W_1^{(1)} h_i^{(1)} + W_2^{(1)} \sum_{j \in \mathcal{N}(i)} W_1^{(0)} h_j^{(0)} + W_2^{(1)} W_2^{(0)} \sum_{k \in \mathcal{N}(\mathcal{N}(i))} h_k^{(0)} + W_2^{(1)} |\mathcal{N}(i)| b^{(0)}  + b^{(1)} \right)\\
    % &\quad = \sigma \left( W_1^{(1)} h_i^{(1)} + W_2^{(1)} \sum_{j \in \mathcal{N}(i)} W_1^{(0)} h_j^{(0)} + W_2^{(1)} W_2^{(0)} \sum_{k \in \mathcal{N}^2(i)} h_k^{(0)} + W_2^{(1)} |\mathcal{N}(i)| b^{(0)}  + b^{(1)}\right) \\
    &\quad = \sigma \left( W_1^{(1)}h_i^{(1)}+ W_2^{(1)}W_1^{(0)}\sum_{j \in \mathcal{N}(i)} h_j^{(0)}+ W_2^{(1)} W_2^{(0)} \sum_{k \in \mathcal{N}^2(i)} h_k^{(0)}  + W_2^{(1)} |\mathcal{N}(i)| b^{(0)} + b^{(1)}\right)
     %  + W_3b^{(0)} + b^{(1)}\right)
     % &\quad = \sigma \left( W_0h_i^{(1)}+ W_1\sum_{j \in \mathcal{N}(i)} h_j^{(0)}+ W_2 \sum_{k \in \mathcal{N}^2(i)} h_k^{(0)}  
     %  + W_3b^{(0)} + b^{(1)}\right)\\
     % &\quad = \sigma \left( W_0h_i^{(1)}+ W_1\sum_{j \in \mathcal{N}(i)} h_j^{(0)}+ W_2 \sum_{k \in \mathcal{N}^2(i)} h_k^{(0)}  
     %  + W_3\right)
\end{align}
where $\mathcal{N}^l(i)$ denotes the set of $l$-hop neighbors of node $i$.

\subsection{GCN without self-loops}
For GCN without self-loops, in Eq. \ref{eq:sum}, its $W_1^{(k)}$ should be 0. Thus its layer-wise propagation output can be expressed as:
\begin{equation}
h_i^{(k+1)} = \sigma \left(  W_2^{(k)} \sum_{j \in \mathcal{N}(i)} h_j^{(k)} + b^{(k)} \right)
% \label{eq:sum}
\end{equation}
Its Node representation after $2$-lay GNN is:
\begin{equation}
     h_i^{(2)} = \sigma \left(   W_2^{(1)} W_2^{(0)} \sum_{k \in \mathcal{N}^2(i)} h_k^{(0)}  + W_2^{(1)} |\mathcal{N}(i)| b^{(0)} + b^{(1)}\right)
\end{equation}
Only 2-hop neighbor information is used to predict the self-node classification.




==> tab/ak.tex <==
\begin{table*}[]
    \caption{non-zero rate and performance of k-order A for datasets. equivalent adjacency matrix quickly get full connection and worse performance with hop increases.}
    \label{tab:ak-smooth}
    \centering
    \begin{small}
    \begin{tabular}{c|c|c|c|c|c}
    & $A$ &  $A^2$ &  $A^3$ &   $A^4$ &  \\
        CiteSeer(in) add selfloop &  \\
           CiteSeer(in) remove selfloop &  \\
         CiteSeer(out) &   \\
        CiteSeer(double) &   \\ 
       CoraML(in) & 
    \end{tabular}
    \end{small}

\end{table*}

==> tab/k_layer_a_1_layer_ak.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab:k-layerA=1-layerAk}
\end{table}
